The dynamics of the TRAPPIST-1 system in the context of its formation

TRAPPIST-1 is an 0.09 $M_{\odot}$ star, which harbours a system of seven Earth-sized planets. Two main features stand out: (i) all planets have similar radii, masses, and compositions; and (ii) all planets are in resonance. Previous works have outlined a pebble-driven formation scenario where planets of similar composition form sequentially at the H$_2$O snowline (${\sim}0.1$ au for this low-mass star). It was hypothesized that the subsequent formation and migration led to the current resonant configuration. Here, we investigate whether the sequential planet formation model is indeed capable to produce the present-day resonant configuration, characterized by its two-body and three-body mean motion resonances structure. We carry out N-body simulations, accounting for type-I migration, stellar tidal damping, disc eccentricity-damping, and featuring a migration barrier located at the disc's inner edge. Due to the sequential migration, planets naturally form a chain of first-order resonances. But to explain the period ratios of the b/c/d-system, which are presently in higher-order resonances, we find that planets b and c must have marched across the migration barrier, into the gas-free cavity, before the disc has dispersed. We investigate both an early and late cavity infall scenario and find that the early infall model best matches the constraints, as well as being more probable. After the dispersal of the gaseous disc, stellar tidal torque also contributes towards a modest separation of the inner system. We outline how the insights obtained in this work can be applied to aid the understanding of other compact resonant planet systems.

==> reply2.tex <==
Dear editor and referee,

we thank the referee for their positive comments. We have addressed the remaining few issues raised by the referee and editor. See below.

Best regards,
Shuo Huang and Chris Ormel.


> Assistant editor comments;
> Please move Figure A1 out of the References and into the Appendix 
Addressed. Thanks!

> Reviewer's Comments:
> Reviewer: 1

>>> Firstly, some of the parameters are significantly different from those used in previous studies. For example, they require a strong eccentricity damping (C_e=0.1 in Fig.14), which is 10 times stronger
than the value estimated from the linear analysis (C_e=1.28). It is true that C_e~0.1 is suggested in Cresswell et al. (2006), but Cresswell et al. use C_e=1.28 in later publications (e.g., Cresswell
et al. 2008), which is consistent with their 3D fluid simulation. I also do not think that the reason why the eccentricity damping is 40 times larger near the cavity (A_e=40) is properly justified. A_e=40
and C_e=0.1 together make the eccentricity damping 400 times stronger, and I do not readily believe that such a condition can be achieved.

>> In the old model (Figure 10.) we saw that the likelihood of success is highest for high A_e. We were encouraged by recent N-body simulations (Atteiee et al. 2020) that indicated such enhanced damping and we indeed speculated that a gas pileup, related to magnetospheric accretion, may operate to enhance the eccentricity damping. But we agree with the referee that it may be stretching the model. We have addressed this point in the second paragraph in section 7.1.

> I think this has been properly described as a problem.

Addressed.

>> Regarding the eccentricity-to-semi-major axis damping parameter C_e, we consistently find (Figs. 8, 10, 14) that the results are more in line with the observations when this parameter is low, so this is a
conclusion of our work. One possibility is that the Type-I migration rate is (for some reason) weaker than the linear formula, i.e., our \gamma_I parameter is small.

> It would be good to elaborate more on why \gamma_I is small. The possibility of small \gamma_I in relation to the torque is mentioned in Section 2.3. It would be good if the authors comment, for example, on the possibility of realizing small \gamma_I with different disk models.

Addressed. We have added a few more sentence in Sect. 2.3, to assess the condition of the protoplanet disks that feature small \gamma_I. We also highlight our finding on small \gamma_I in Sect. 8.

>> Secondly, I do not understand the physics behind some of the settings. In particular, it is not explained why the disc force (F_disc) for planets b and c is suddenly switched off. Why do planets b-c go through the disc edge and why not planet d? It is stated that the timing of migration of planet c and the timing of disc dispersal
could be simultaneous. However, given the migration time-scale (~10 kyr) and disk lifetime (~1 Myr), it is quite difficult for these to be simultaneous. In addition, the timing of the input of the planet g is quite arbitrary, as mentioned in several places in the paper.

>> We do indeed need planets b and c to fall in the cavity, as we can otherwise not explain the resonance structure (Section 3), a conclusion that is consistent with other works (e.g., Papaloizou et al. 2018). We do not provide a quantitative model for the infall of these planets; it is indeed a model Ansatz (assumption). But we do present motivations. In our old model (Section 4) we postulated that the infall may coincide with the decay of the disk, the disk becomes thinner therefore corotation torque on planet b and c cannot support outer planets in the disk. In the new model (Section 5), we imagine that planet b and c excavate gaps, while planet d, being smaller,
does not. Modelling how these processes would operate in detail, is beyond the scope of this work.

> I understand that only planets b-c go through the edge is the model assumption. Explanations on this point have been added to the manuscript. For the late infall model, the authors answered "we postulated that the infall may coincide with the decay of the disk", but it seems difficult given that the migration timescale is shorter than the disk dissipation timescale. In that sense, the early infall model might be better. Since there are other ways for planets to enter the inner cavity during the migration phase (Stage I) than the one described by the authors (i.e., gap opening), the early infall model seems more achievable.

We agree. In the discussion section we evaluate the late infall and early infall models in detail. Although there are other possibilities for explaining the model setting of late infall model, such as planet b and c growing large enough that they open gaps and enter the disk cavity, the early infall model is more straightforward. 

>>> In summary, the authors deserve credit for finding a scenario that explains the resonant configuration of the TRAPPIST-1 system. However, I am not convinced that this will occur with any realistic probability. Rather, they may conclude that it would be very difficult to reproduce the resonant configuration of the TRAPPIST-1 system. I hope the authors do more to justify their settings and assumptions or discuss them as caveats.

>> We hope that the revised manuscript provides more insight in the model design. We think that we have implemented relatively simple model design choices and offer neutral assessment by conducting parameter surveys. As said above, we do agree with the referee that the old model is somewhat unlikely. The new setup is in our view
plausible.

> I agree. I think the model is simpler now. 

Thanks!
